Optimal Transfer Learning for Missing Not-at-Random Matrix Completion

We study transfer learning for matrix completion in a Missing Not-at-Random (MNAR) setting that is motivated by biological problems. The target matrix $Q$ has entire rows and columns missing, making estimation impossible without side information. To address this, we use a noisy and incomplete source matrix $P$, which relates to $Q$ via a feature shift in latent space. We consider both the active and passive sampling of rows and columns. We establish minimax lower bounds for entrywise estimation error in each setting. Our computationally efficient estimation framework achieves this lower bound for the active setting, which leverages the source data to query the most informative rows and columns of $Q$. This avoids the need for incoherence assumptions required for rate optimality in the passive sampling setting. We demonstrate the effectiveness of our approach through comparisons with existing algorithms on real-world biological datasets.

==> 2.prelim.tex <==
\section{Transfer Learning via Spectral Features}







\subsection{From entry-wise guarantees to spectral features}

\begin{prop}\label{prop:spectral-features}
    Let $P$ an $m \times n$ matrix of rank $r$. Let $\epsilon > 0$, and  $\widehat{P}$ be a rank-$r$ estimate of $P$, satisfying 
    \begin{align}
        \Vert \widehat{P} - P \Vert_{\max} \le \epsilon \Vert P \Vert_{\max}.
    \end{align}
    Consider the SVDs $P = U \Sigma V^\top$, and $\widehat{P} = \widehat{U} \widehat{\Sigma} \widehat{V}^\top$.
    Then, it holds that
    \begin{align*}
        & \min_{W \in \cO^{r \times r}}\Vert U - \widehat{U} R\Vert_{2 \to \infty}  \\
        & \qquad \le \frac
        {(2\sqrt{n} + (2+\sqrt{2}) \sqrt{mn}\Vert UU^\top \Vert_{2 \to \infty}  
  ) \Vert  P -  \widehat{P} \Vert_{\max}}{\sigma_r(P)}\\
         & \min_{W \in \cO^{r \times r}}\Vert V - \widehat{V} W\Vert_{2 \to \infty}  \le  \\
         & \qquad  \le \frac
        {(2\sqrt{m} + (2+\sqrt{2}) \sqrt{mn}\Vert VV^\top \Vert_{2 \to \infty}  
  ) \Vert  P -  \widehat{P} \Vert_{\max}}{\sigma_r(P)}
    \end{align*}
    provided that 
    \begin{align*}
        \sqrt{mn} \Vert \widehat{P} - P \Vert_{\max} \le \sqrt{mn} \epsilon \Vert P \Vert_{\max} \le \frac{\sigma_r(P)}{2} 
    \end{align*}
\end{prop}

\yj{The proof is given the appendix?}

\yj{The above results allows us to deduce subspace recovery guarantees in the two-to-infinity norm so long as we have tight control on the entry-wise estimation guarantee of $\widehat{P}.$}


We hypothesis that we have access to an estimate $\hat{P}$ that satisfies the conditions of the proposition above. Our reasoning for assuming such hypothesis is giving below



\yj{Recent progress in matrix completion in  the MNAR and MCAR setting have established entry-wise guarantees under various conditions and assumptions. Below, we give examples that provide such guarantees:}

\yj{Examples: 
\begin{itemize}
    \item Entry-wise guarantees in the MCAR setting for noisy matrix completion \cite{chen2020noisy}
    \item Entry-wise guarantees in the MNAR setting: we can cite Dev's papers \cite{agarwal2023causal} and the one I had \cite{jedra2023exploiting}
    \item We can conjecture that  Deep Learning methods can lead to low entry-wise errors (Foundational models for tabular data + Large Graph neural networks, often used for this kind of settings)
\end{itemize}
}


\subsection{Regression with Spectral Features}

\yj{After that we can describe the regression with spectral features. More precisely if $i,j \in \Omega_Q$ (here I am denoting $\Omega_Q$ the set of observed features.)
\begin{align*}
    A_{Q,i,j} & = Q_{ij} + (A_{Q,i,j} - Q_{ij}) \\
    & = \hat{u}_i^\top \Theta_Q \hat{v}_j + \underbrace{\epsilon_{ij}}_{\text{misspecification } \hat{P}} + \underbrace{(A_{Q,i,j} - Q_{ij})}_{noise}
\end{align*}
where $\Theta_Q = R \Sigma_Q L $ where $L$ and $Q$ are unknown rotations due the shift. We clarify what values $\epsilon_{ij}$ and $\Theta_Q$ is below:
}


\yj{Below, we can write an error decomposition with Least squares}
We define the LSE as 
\begin{align*}
    \hat{\Theta}_Q \in \arg\min_{\Theta \in \mathbb{R}^{r \times r}} \sum_{i,j \in \Omega_{Q}} \vert  A_{Q,i,j}  - \hat{u}_i^\top \Theta \hat{v}_j  \vert^2 
\end{align*}
where $\Omega_Q$ is the set of observed entries $(i,j) \in \Omega$. Then, we use the estimate $\hat{\Theta}_Q$ to predict the unobserved entries: $\forall (i,j) \in ([m]\times[n]) \backslash \Omega_Q$:  
\begin{align*}
    \hat{Q}_{ij} = \hat{u}_i^\top \hat{\Theta} \hat{v}_j 
\end{align*}
The quality of this predictors depends on the quality of $\hat{U}$ and $\hat{V}$ as well as the set of observed entries $\Omega_Q$. Below we characterize how is this dependence:
\begin{lemma}[Error Decomposition]
    \begin{align*}
        \vert \hat{Q}_{ij} - Q_{ij} \vert  \le 
    \end{align*}
\end{lemma}





